Flux-Matched Poisson Iteration for Generated Jacobian Equations: Local Convergence and Spectral Galerkin Approximation

We develop a flux-matched Poisson iteration for solving generated Jacobian equations with second boundary conditions. In each step, it solves a fixed shifted Poisson problem with a Neumann-type boundary condition. Near a smooth regular solution with positive $C^{1,1}$ densities, we prove that the iteration has local geometric convergence in $C^{2,\alpha}$ on smooth connected Riemannian domains. The iteration is then discretized using a spectral Galerkin method, with local convergence proved for the Fourier-Jacobi scheme on spherical caps. Optical numerical experiments support these estimates and demonstrate useful imaging performance beyond the local convergence theory.

==> data_adjacent/imaging_summary.tex <==
Far letter A & 26 & 7.15 & 99.987 & 0.1200 & 0.0217 & 8.51 & 2.89 \\
Far two regions & 20 & 8.43 & 99.983 & 0.1315 & 0.0257 & 6.57 & 2.35 \\
Near letter A & 177 & 8.28 & 94.435 & 0.1384 & 0.0158 & 50.39 & 5.30 \\
Near complex & 115 & 12.90 & 96.347 & 0.1801 & 0.0239 & 32.71 & 3.80 \\


==> data_adjacent/refractor_results.tex <==
Gaussian spots & 91 & $8.91\times10^{-11}$ & $7.92\times10^{-11}$ & $7.91\times10^{-11}$ & $0.701$ \\
ZJU, 1 px & 27 & $3.57\times10^{-3}$ & $2.72\times10^{-4}$ & $3.57\times10^{-3}$ & $0.686$ \\


==> data_adjacent/sigma.tex <==
0 & 35 & 1.297 & 46 & 6.339 \\
1 & 35 & 1.304 & 53 & 3.678 \\
5 & 36 & 13.254 & 82 & 7.970 \\


==> data_adjacent/smooth_validation.tex <==
Near & 8 & 44 & 15 & $2.49\times10^{-2}$ & $2.51\times10^{-3}$ \\
Near & 12 & 90 & 35 & $3.15\times10^{-5}$ & $2.20\times10^{-6}$ \\
Near & 16 & 152 & 61 & $5.56\times10^{-9}$ & $2.96\times10^{-10}$ \\
Far & 4 & 14 & 10 & $3.37\times10^{-2}$ & $5.96\times10^{-3}$ \\
Far & 8 & 44 & 24 & $8.84\times10^{-5}$ & $8.73\times10^{-6}$ \\
Far & 14 & 119 & 62 & $1.85\times10^{-10}$ & $1.27\times10^{-11}$ \\

